Deriving and Validating Requirements Engineering Principles for Large-Scale Agile Development: An Industrial Longitudinal Study

In large scale agile systems development, the lack of a unified requirements engineering (RE) process is a major challenge, exacerbated by the absence of high level guiding principles for effective requirements management. To address this challenge, we conducted a five year longitudinal case study with Grundfos AB, in collaboration with the Software Centre in Sweden. RE principles were first derived through qualitative data collection spanning more than 25 sprints, approximately 320 weekly synchronisation meetings, and seven cross-company, company-specific workshops between 2019 and 2024. These activities engaged practitioners from diverse roles, representing several hundred developers across domains. In late 2024, five in depth focus groups with senior leaders at Grundfos provided retrospective validation of the principles and assessed their strategic impact. We aim to (1) empirically examine RE principles in large scale agile system development, (2) explore their benefits in practice within the case company, and (3) identify a set of transferable RE principles for large scale contexts. Using thematic analysis, six key RE principles architectural context, stakeholder-driven validation and alignment, requirements practices in large-scale agile organisations. evolution with lightweight documentation, delegated requirements management, organisational roles and responsibilities, and a shared understanding of requirements are derived. The study was further validated through crosscompany expert evaluation with three additional multinational organisations (Bosch, Ericsson, and Volvo Cars), which are directly responsible for largescale requirements management. Together, these efforts provide a scalable and adaptable foundation for improving requirements practices in largescale agile organisations.

==> figure/_archive/03_usecase.tex <==
\subsubsection*{Use case}
If the context of a use case is of importance, one first needs to establish a common understanding of what encompasses a use case. Figure~\ref{fig:RE_UseCases} shows the themes identified in regards to the use case definition given by the interviewees.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/RE_UseCase.pdf}
    \caption{Themes in regards to the definition of use case}
    \label{fig:RE_UseCases}
\end{figure}

In brief summary, the use case is supposed to be an easy and effective way of communicating the desired system behaviour on a high level between stakeholders of that system. Several interviewees reflect that for automatic driving systems the use case contains information about the context in which the system is supposed to operate (e.g. in form of an automation level). The use case should be specific enough to ease the definition of tests. This includes enough information about the context to allow for defining and reproducing clear test cases for the desired behaviour in the desired context.

==> figure/_archive/04_results.tex <==
%An interviewee suggested to describe the context by looking at different aspects, for example a context for the users, a context for the actors, and a context for the entire system. The context of the users in an automatic vehicle for example would be the ability of the users to take over the vehicle in case the automatic function fails (e.g. driving license of the user). The context of the actors would be the state of entities that are directly or indirectly influenced by the system (e.g. other road users). The context of the system is the operational condition in which the system operates (e.g. state of the road, state of the vehicle's systems). 
%\paragraph{What defines the context?} All interviewees stated that knowledge about the context is important for validation, safety, and security of the system. If assumptions about the context of a system are made, they need to be clearly communicated as assumptions. %Therefore, the context should be in some form properly defined. One problem an interviewee mentioned with defining what context actually means are assumptions: If assumptions about the context of a system are made, they need to be clearly communicated as assumptions. An example mentioned is the assumption for an automatic driving system that pedestrians do not occur on a motorway. Although laws forbidding pedestrians on motorways in most countries support this assumption, there remains a small prop ability that pedestrians do occur in the context of a motorway, which needs to be taken into account or at least stated as residual risk for a system failure for this context assumptions.

==> figure/_archive/07_Conclusion_and_future_work_.tex <==
\section{Conclusion and future work}
The study aimed to identify effective approaches and challenges in requirement representation for automotive perception systems, focusing on whether a shared language could address these challenges without disrupting successful methods. Interviews revealed a need for industry standards in ML development, with effective approaches combining natural language requirements and ODDs. Multi-party communication involved trade-offs, and fairness was implicit in safety and performance standards. The study suggests that shared language could help, though concerns about sharing sensitive information persist. Future research could assess the impact of shared language and evaluate the role of the \emph{ISO/CD PAS 8800 standard}.

==> figure/_archive/20210505_03_Framework.tex <==
\section{A compositional system architecture framework}
\begin{itemize}
    \item Designing a large, distributed system is a hierarchical process \cite{Murugesan2019}. 
    \item In a hierarchical design process for a large system, it will be necessary to establish several views on the overall system in order to factor the design task into smaller and specialised tasks.
    \item Zardini et al. show how co-design of hardware and software can be modelled with category theory for an autonomous driving function \cite{Zardini2020}.
    \item We establish a framework to describe how the connection between different views on a large scale architecture can be described with category theory. Furthermore, category theory establishes a suitable description of the abstraction levels on each view and it links viewpoints on each abstraction level together. 
\end{itemize}

\subsection{Architectural views as objects in categories}
Figure \ref{fig:03_ArchViewpasorder} shows exemplified three aspects of a system: Logical Behaviour, Hardware, and Cybersecurity. Each box represents a view governed by an architecture viewpoint on the final system. Note that, for each aspect, the level of details increases the further the evolution of the system design proceeds. Let us call the levels, from top (highest abstraction) to bottom (highest level of detail), analytical level, conceptual level and design level. For each aspect of the system, we obtain a \emph{partially ordered set} (poset) of views:
\begin{proposition}
The architectural views of a system aspect form a partially ordered set.
\end{proposition}
\begin{proof}
Let $a$, $b$, and $c$ be architectural views. It always holds that an architectural view is related to itself ($a\leq a$, reflexivity). If $a$ is of less or equal detail than $b$, and $b$ is of less or equal detail than $c$, then $a$ must be of less detail than $c$ (transitivity). Finally, if $a$ is of less or equal detail than $b$, and $b$ is of less or equal detail than $a$, then $a$ and $b$ must be of equal detail (antisymmetry).
\end{proof}

"A category is a collection of objects which are related to each other in a consistent way" \cite{Perrone2021}. 

\begin{proposition}
The partially ordered set of architectural views describing a system aspect can be seen as a category:
\end{proposition}
\begin{definition}
The category $\mathbf{C_{sa}}$ describing a system aspect has architectural views as its objects. Given two architectural views $a$ and $b$, then $\text{Hom}_\text{sa}(a,b) = {(a,b)}, \text{if}\; x\leq y$ describes the morphisms between architectural views of different levels of abstractions. The identity morphism is the identify function mapping an architectural view to itself. Furthermore, given an additional architectural view $c$, and defining the morphism $g\in \text{Hom}_\text{sa}(a,b)$ and $f\in \text{Hom}_\text{sa}(b,c)$, there exists a morphism $f \text{;} g$ such that the composition of $f$ and $g$ is $\text{Hom}_\text{sa}(a,c)$.
\end{definition}



An system architecture description consists of one or more architectural views.
\begin{definition}
A function $f: X\rightarrow Y$ for which elements $a, b \in A$
\end{definition}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{figs/Arch-CoDesign.pdf}
    \caption{Order of Architecture Viewpoints}
    \label{fig:03_ArchViewpasorder}
\end{figure}

\begin{definition}

\end{definition}


The objects in that category are 

\subsection{Dependencies between categories}

\emph{Idea: A functor is a mapping preserving or respecting the relations between the objects \cite{Perrone2021}.}

\subsection{Enabling traceability}

\subsection{Verification and validation}

==> figure/_archive/20210930_04_Results_____Kopi.tex <==
\section{Results}
This section presents the results based on the data obtained through the interview sessions. 
The section is divided into subsections presenting each research questions individually because the research questions built upon each other. 

\subsection{RQ1: What is the current understanding of context definitions?}
The first 15 minutes of the interviews were used to establish an overview of the interviewee's understanding of the terms context and ODD. 

\paragraph{What is context?} The interviewees were asked to elaborate on their understanding of what is meant by context definition (in relation to automatic driving / advanced driver assistance). 
Thirteen interviewees were unsure what context definition describes in relation to automatic driving systems.
Two interviewees considered the context definition and ODD to be identical in that they both describe environmental conditions in which the system is designed to operate:

\begin{tcolorbox}
“[...] it’s kind of the same things as the ODD is describing but context contains all the possible combinations, if you like, of where this is going to operate.”
\end{tcolorbox}

Most interviewees did not see context and ODD as identical definitions. 
Instead they stated that the ODD is a subset of the context derived from use cases. 
%However, one interviewee describes the context to be a specific scenario within the ODD, or discrete points in the ODD. 
%The ODD would then represent the sum of all those discrete points, i.e., contexts:

%\begin{tcolorbox}
%"[...] it's almost like to say it's discrete points in the ODD if you want this really specific conditions that you define %around a use case."
%\end{tcolorbox}

\paragraph{What entails the context?} All interviewees describe the context as a dynamic, and rather wide entity, that should include situations, scenarios, and the environments in which a system operates.
\begin{tcolorbox}
"But it is a way to define a situation, or define a system, or defining [...] a scenario, or an environment [...]. So that is what I would call a context."
\end{tcolorbox}
One interviewee includes also the functional state of the vehicle in the context.
All interviewees stated that knowledge and a clear description about the context is important for validation, safety, and security of the system. 
If assumptions about the context of a system are made, they need to be clearly communicated as assumptions.

\subsubsection*{Operational Design Domain (ODD)}

\paragraph{What is the ODD?} All interviewees agreed with SAE J3016 definition of the ODD \cite[Page 14]{SAE2018}. 
Although SAE J3016 provides a definition of the ODD, all interviewees mention that there is lack of standardisation of the format of an ODD. 
A majority of interviewees added that a description of a design domain beyond the actual ODD, in which the system's performance is degraded but still safe, is necessary in addition to the ODD.

\begin{tcolorbox}
"[...] in the ODD you have to describe it as sort of a graceful degradation of the system when you go outside it's never included".
\end{tcolorbox}

\paragraph{What entails the ODD?} A majority of interviewees claimed that the SAE definition is incomplete. 
A major missing aspect that was mentioned is the internal state of the vehicle, i.e., capability of sensors and actors.
Furthermore, the drivers' behaviour in and around the vehicle should be described in the ODD (e.g. can the system operate with an intoxicated or distracted driver?). 
Ten interviewees reminded that the road and lane conditions should explicitly be highlighted in the ODD, as they play a major role in the correct function of automatic driving systems. 

\paragraph{What is the difference between context and ODD?} ODD is by all interviewees associated with safety and performance guarantees. The context is associated with validity of requirements derived from a given use case. If one views the context definition as a form of world description\footnote{analogue to the World-Machine Model described by Jackson in \cite{Jackson1995}}, the ODD is an abstraction of the context in which a given system can testable operate with desired characteristics, such as safety, reliability, and performance. 

\subsection{RQ2: What are the challenges with deriving context definitions from use cases?} \label{subsec:RQ2}
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{figs/RE_RQ1_Overview.pdf}
%    \caption{Areas of challenges when deriving contextual definitions from use cases.}
%    \label{fig:RE_RQ1_Overview}
%\end{figure}
This section describes the major challenges through themes identified from the interviews. Three areas of challenges illustrated were identified from the interview sessions and validated by the focus group. They are "deriving context definitions", "process, responsibility, and communication of context definition", and "deriving the ODD from context definition". For each area of challenge, only the themes validated with a simple majority by the focus group members are presented. The areas of challenges and themes voted out by the focus group are collected in \cite{Linder2021}.

\subsubsection{Deriving context}
Table \ref{tab:Deriving context} provides the validated themes and brief descriptions regarding the challenges associated with deriving context definitions from use cases.
\begin{table}[h]
\centering
\caption{Themes relates to challenges with deriving context definitions.}
\label{tab:Deriving context}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
Lack of standard & A common language for context definitions is lacking, which makes it difficult to work on a system or product in different countries, companies, or even teams. Unlike requirement specification, there is no correspondent context specification, which results in ambiguities in the context in which requirements are valid.\\
\rowcolor[HTML]{EFEFEF} 
Difficult to describe context & There is a lack of terminology for describing non-numeric parameters within the context, like the weather: It is for example not clear what "in good weather conditions" actually means. Therefore, non-numeric parameters are difficult to compare between different context descriptions. Furthermore, the environment is often dynamic and containing unknown unknowns, which can change the context of a system unpredictably. \\
Validity range of the context & A lack of transparency in use case creation and requirement negotiation leads to challenges when defining the desired and feasible context of the system. It is seen as important that the function developers obtain more knowledge about the use case in order to understand the necessary context in which a function / system shall operate. Furthermore, it was stated that there is no good practise in determining if a system still operates within its designated context. \\
\hline
\end{tabular}
\end{table}
\FloatBarrier

\subsubsection{Process, responsibility, and communication}
Table \ref{tab:Process, responsibility, and communication} provides the validated themes and brief descriptions regarding the challenges associated with the process, responsibility, and communication of context definitions.
\begin{table}[h]
\centering
\caption{Themes related to challenges with the process, responsibility, and communication of context definitions.}
\label{tab:Process, responsibility, and communication}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}c}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
Lacking involvement of function developers & Function developers are detached from the overall picture, because they are not involved enough in defining requirements and context definitions. This makes it hard for them to understand the context in which the system is supposed to function. \\
\rowcolor[HTML]{EFEFEF} 
Misinterpretation of requirements & Textual requirements and context definitions can be misinterpreted by different peoples with different views on the system. Often, the person writing the requirements and context definitions has no direct contact to the person implementing them. \\
Assumptions not documented & A main concern mentioned was that assumptions about the context and in the requirements are not being properly documented as such. In many cases it is necessary to make assumptions, but they must be clearly documented as such. A typical context assumption for a function is to assume a linear behaviour of some measured dynamic. \\
\rowcolor[HTML]{EFEFEF} 
Difficult process & The process of deriving contextual information and requirements from use cases was described as being "blurry and unsharp by nature". It was also mentioned, that a common structured process is either missing or too complex for deriving both requirements and context definitions. \\
Lack of feedback loop & Sometimes changes in the context, and even requirements, of a system are only discovered during the development. A feedback loop is often missing to verify if these changes in context are acceptable. \\
\hline
\end{tabular}
\end{table}
\FloatBarrier

\subsubsection{Defining ODD}
Table \ref{tab:ODD} provides the validated themes and brief descriptions regarding the challenges associated with defining an ODD out of the context definition.
\begin{table}[h]
\centering
\caption{Themes related to challenges with defining the ODD.}
\label{tab:ODD}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
No standard way of defining ODD & ODD tents to mean different things, which makes it difficult to understand what an ODD shall entail. Different OEMs, and even different teams within an OEM, have different approaches to define the ODD, which creates confusion for Tier 1 suppliers. The lack of a standardisation has been mentioned by all interviewees as a major obstacle.\\
\rowcolor[HTML]{EFEFEF} 
Difficult to capture all scenarios in ODD & To enumerate all possible scenarios in the ODD is impossible. It is difficult to determine, which scenarios the ODD should entail, and which scenarios are not required to be captured by the ODD.\\
Hard to model ODD & Especially "edge case" scenarios are difficult to describe in the ODD, because many assumptions are necessary in these scenarios, which are often not well documented in the context description. \\
\rowcolor[HTML]{EFEFEF} 
Hard to understand context definitions & Function developers are not always involved in defining the context definitions, which makes it difficult for them to develop an ODD that fits the desired context.   \\
Overly cautious & A consequence of not knowing the right context of the system is that the ODD will be overly cautious. Developers will start with a too strict and too limited ODD, and only expand it once safety has been proven within small extensions. This can lead to unnecessary long developing and testing times, or overly cautious systems.\\
\rowcolor[HTML]{EFEFEF} 
Arguing for completeness & It is difficult to know when an ODD captures all relevant scenarios and elements, mainly because there is no standardised method or template for determining if the ODD is complete. \\
\hline
\end{tabular}
\end{table}
\FloatBarrier

\subsection{RQ3: Which support would be appropriate for deriving context definitions from use cases?}
For each of the three areas of challenges described in Section \ref{subsec:RQ2} the interviewees were asked to suggest improvements. Out of the interviews, themes were identified and presented to the focus group for validation. All themes that achieved a simple majority vote in the focus group are presented in this section. 


\subsubsection{Improvement ideas for deriving context definitions}
Table \ref{tab:Improvements_Derivingcontext} provides the validated themes and brief descriptions regarding the improvement ideas for deriving context definitions.
\begin{table}[h]
\centering
\caption{Themes related to improvement ideas for deriving context definitions.}
\label{tab:Improvements_Derivingcontext}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
Diversity of sensor data & According to one interviewee, a more diverse set of sensor data of the environment allows for easier interpretation and limitation of the context in which the system operates.\\
\rowcolor[HTML]{EFEFEF} 
Knowing prerequisites & According to one interviewee, an improvement would be to have a clearer understanding of prerequisites for the different use cases. For example, prerequisites could entail existence of special infrastructure for automatic driving, such as smart roads or low latency high bandwidth mobile data connections. \\
Standardised approach & All interviewees suggested to standardised context definition to ease cooperation between different teams and companies.  \\
\hline
\end{tabular}
\end{table}
\FloatBarrier

\subsubsection{Improvement ideas for the process, responsibility, and communication}
Table \ref{tab:Improvements_Process} provides the validated themes and brief descriptions regarding the improvement ideas for the process, responsibility, and communication of context definitions.
\begin{table}[h]
\centering
\caption{Themes related to improvement ideas for the process, responsibility and communication of context definitions and ODDs}
\label{tab:Improvements_Process}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
Involve function developers & Function developers should be more involved in the requirement engineering process, including context definition and deriving the ODD. On one hand, the function developers would get a better understanding of the requirements and context. On the other hand, they can contribute with deep knowledge about the used technologies, which eases the understanding of the the technology's capability for desired contexts. \\
\rowcolor[HTML]{EFEFEF} 
Continuous improvement & Automatic driving is a new technology, which needs to evolve continuously. The processes for deriving relevant artefacts, such as the context definition and ODD need to evolve together with the technology. \\
\rowcolor[HTML]{EFEFEF} 
Faster loops & One suggested improvement was to derive requirements faster, and creating faster feedback loops between the stakeholders. This expedites also the definition of the context, because assumptions can be made and verified faster. \\
Leveraging from other contexts & Typically automatic driving systems are developed for and tested in confined areas, such as factory areas or harbours. Lessons are learnt in these confined contexts, and it is important to be able to leverage the knowledge from these confined contexts into new contexts. \\
\rowcolor[HTML]{EFEFEF} 
Integrate requirement engineering better into SAFe setup & It is perceived that requirement engineering is not well integrated in scaled agile frameworks (SAFe), which hinders an efficient development and handling of requirements, and consequently context definitions.\\
\hline
\end{tabular}
\end{table}
\FloatBarrier

\subsubsection{Improvement ideas for defining ODD}
Table \ref{tab:Improvements_ODD} provides the validated themes and brief descriptions regarding the improvement ideas for defining the ODD out of a context definition.
\begin{table}[h]
\centering
\caption{Themes related to improvement ideas for defining the ODD.}
\label{tab:Improvements_ODD}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
Criteria for knowing that ODD is complete & One interviewee suggested that an explicit method and criteria are needed to proof that the ODD is complete and correct. \\
\rowcolor[HTML]{EFEFEF} 
Standardised approach & All interviewees suggest to improve on standardisation for defining ODD. \\
Automatic tool for deriving ODD & The described improvement would encompass a tool that can take as input the context, requirements based on the context and test cases. It would then propose an appropriate ODD, that is valid in the desired context, entails all requirements, and is verified through test cases. \\
\rowcolor[HTML]{EFEFEF} 
Information should be described clearly in ODD &  The ODD should contain more information about the context of the system. According to one interviewee, this would improve identifying wrong assumptions about the context early. \\
Measure of exposure to a safety event & One interviewee explained that the hazard and risk assessment to evaluate the dimensions of the ODD from a safety viewpoint. The HARA includes assumptions about the context, and especially the exposure to a hazardous context can then be used to decide on the ODD. \\
\hline
\end{tabular}
\end{table}
\FloatBarrier

==> figure/_archive/20211005_04_Results.tex <==
\section{Results}
This section presents the results based on the data obtained through the interview sessions. 
The section is divided into subsections presenting each research questions individually because the research questions built upon each other. 

\subsection{RQ1: What is the current understanding of context definitions?}
The first 15 minutes of the interviews were used to establish an overview of the interviewee's understanding of the terms context and ODD. \par

\noindent \textbf{What is context?} The interviewees were asked to elaborate on their understanding of what is meant by context definition in relation to automatic driving. 
Thirteen interviewees were unsure what context definition describes in relation to automatic driving systems.
Two interviewees considered the context definition and ODD to be identical in that they both describe environmental conditions in which the system is designed to operate:

\begin{tcolorbox}
\footnotesize
“[...] it’s kind of the same things as the ODD is describing but context contains all the possible combinations, if you like, of where this is going to operate.”
\end{tcolorbox}

\noindent Most interviewees did not see context and ODD as identical definitions. 
Instead they stated that the ODD is a subset of the context derived from use cases. \par
%However, one interviewee describes the context to be a specific scenario within the ODD, or discrete points in the ODD. 
%The ODD would then represent the sum of all those discrete points, i.e., contexts:

%\begin{tcolorbox}
%"[...] it's almost like to say it's discrete points in the ODD if you want this really specific conditions that you define %around a use case."
%\end{tcolorbox}

\noindent \textbf{What entails the context?} All interviewees describe the context as a dynamic, and rather wide entity, that should include situations, scenarios, and the environments in which a system operates.

\begin{tcolorbox}
\footnotesize
"But it is a way to define a situation, or define a system, or defining [...] a scenario, or an environment [...]. So that is what I would call a context."
\end{tcolorbox}

\noindent One interviewee includes also the functional state of the vehicle in the context.
All interviewees stated that knowledge and a clear description about the context is important for validation, safety, and security of the system. 
If assumptions about the context of a system are made, they need to be clearly communicated as assumptions. \par

\noindent \textbf{What is the ODD?} All interviewees agreed with SAE J3016 definition of the ODD \cite[Page 14]{SAE2018}. 
Although SAE J3016 provides a definition of the ODD, all interviewees mention that there is lack of standardisation of the format of an ODD. 
A majority of interviewees added that a description of a design domain beyond the actual ODD, in which the system's performance is degraded but still safe, is necessary in addition to the ODD. \par

\begin{tcolorbox}
\footnotesize
"[...] in the ODD you have to describe it as sort of a graceful degradation of the system when you go outside it's never included".
\end{tcolorbox}

\noindent \textbf{What entails the ODD?} A majority of interviewees claimed that the SAE definition is incomplete. 
A major missing aspect that was mentioned is the internal state of the vehicle, i.e., capability of sensors and actors.
Furthermore, the drivers' behaviour in and around the vehicle should be described in the ODD (e.g. can the system operate with an intoxicated or distracted driver?). 
Ten interviewees reminded that the road and lane conditions should explicitly be highlighted in the ODD, as they play a major role in the correct function of automatic driving systems. \par

\noindent \textbf{What is the difference between context and ODD?} ODD is by all interviewees associated with safety and performance guarantees. The context is associated with validity of requirements derived from a given use case. If one views the context definition as a form of world description\footnote{analogue to the World-Machine Model described by Jackson in \cite{Jackson1995}}, the ODD is an abstraction of the context in which a given system can testable operate with desired characteristics, such as safety, reliability, and performance. 

\subsection{RQ2: What are the challenges with deriving context definitions from use cases?} \label{subsec:RQ2}
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{figs/RE_RQ1_Overview.pdf}
%    \caption{Areas of challenges when deriving contextual definitions from use cases.}
%    \label{fig:RE_RQ1_Overview}
%\end{figure}
This section describes the major challenges through themes identified from the interviews. Three areas of challenges illustrated were identified from the interview sessions and validated by the focus group. They are "deriving context definitions", "process, responsibility, and communication of context definition", and "deriving the ODD from context definition". For each area of challenge, only the themes validated with a simple majority by the focus group members are presented in Table \ref{tab:Challenges}.

\begin{table}[t]
\centering
\scriptsize
\caption{Themes relates to challenges with deriving context definitions.}
\label{tab:Challenges}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
\multicolumn{2}{l}{\cellcolor[HTML]{656565}\color[HTML]{FFFFFF}Deriving context definitions} \\
\textbf{Difficult to describe context} & There is a lack of terminology for describing non-numeric parameters within the context, like the weather: It is for example not clear what "in good weather conditions" actually means. Therefore, non-numeric parameters are difficult to compare between different context descriptions. Furthermore, the environment is often dynamic and containing unknown unknowns, which can change the context of a system unpredictably. \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Lack of standard} & A common language for context definitions is lacking, which makes it difficult to work on a system or product in different countries, companies, or even teams. Unlike requirement specification, there is no correspondent context specification, which results in ambiguities in the context in which requirements are valid.\\
\textbf{Lack of transparency} & A lack of transparency in use case creation and requirement negotiation leads to challenges when defining the desired and feasible context of the system. It is seen as important that the function developers obtain more knowledge about the use case in order to understand the necessary context in which a function / system shall operate. Furthermore, it was stated that there is no good practise in determining if a system still operates within its designated context. \\
\hline
\multicolumn{2}{l}{\cellcolor[HTML]{656565}\color[HTML]{FFFFFF}Defining ODDs} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Lack of arguments for completeness} & It is difficult to know when an ODD captures all relevant scenarios and elements, mainly because there is no standardised method or template for determining if the ODD is complete. \\
\textbf{Difficult to capture all scenarios in ODD} & To enumerate all possible scenarios in the ODD is impossible. It is difficult to determine, which scenarios the ODD should entail, and which scenarios are not required to be captured by the ODD. Especially "edge case" scenarios are difficult to describe in the ODD, because many assumptions are necessary in these scenarios, which are often not well documented in the context description. \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Hard to understand context definitions} & Function developers are not always involved in defining the context definitions, which makes it difficult for them to develop an ODD that fits the desired context.   \\
\textbf{Lack of standard for ODD} & ODD tents to mean different things, which makes it difficult to understand what an ODD shall entail. Different OEMs, and even different teams within an OEM, have different approaches to define the ODD, which creates confusion for Tier 1 suppliers. The lack of a standardisation has been mentioned by all interviewees as a major obstacle.\\
\rowcolor[HTML]{EFEFEF} 
\textbf{Overly cautious} & A consequence of not knowing the right context of the system is that the ODD will be overly cautious. Developers will start with a too strict and too limited ODD, and only expand it once safety has been proven within small extensions. This can lead to unnecessary long developing and testing times, or overly cautious systems.\\
\hline
\multicolumn{2}{l}{\cellcolor[HTML]{656565}\color[HTML]{FFFFFF}Process and communication} \\
\textbf{Assumption not documented} & A concern mentioned was that assumptions about the context and in the requirements are not being properly documented as such. In many cases it is necessary to make assumptions, but they must be clearly documented as such. A typical context assumption for a function is to assume a linear behaviour of some measured dynamic. \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Insufficient involvement of function developers} & Function developers are detached from the overall picture, because they are not involved enough in defining requirements and context definitions. This makes it hard for them to understand the context in which the system is supposed to function. \\
\textbf{Lack of feedback} & Sometimes changes in the context, and even requirements, of a system are only discovered during the development. A feedback loop is often missing to verify if these changes in context are acceptable. \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Misinterpretation of requirements} & Textual requirements and context definitions can be misinterpreted by different peoples with different views on the system. Often, the person writing the requirements and context definitions has no direct contact to the person implementing them. \\
\textbf{Too difficult process} & The process of deriving contextual information and requirements from use cases was described as being "blurry and unsharp by nature". It was also mentioned, that a common structured process is either missing or too complex for deriving both requirements and context definitions. \\
\hline
\end{tabular}
\end{table}

\subsection{RQ3: Which support would be appropriate for deriving context definitions from use cases?}
For each of the three areas of challenges described in Section \ref{subsec:RQ2} the interviewees were asked to suggest improvements. Out of the interviews, themes were identified and presented to the focus group for validation. All themes that achieved a simple majority vote in the focus group are presented in Table \ref{tab:Improvements}. 

\begin{table}[t]
\centering
\scriptsize
\caption{Themes related to improvement ideas for deriving context definitions.}
\label{tab:Improvements}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{\xc\textwidth}m{\yc\textwidth}}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} \\ \hline
\multicolumn{2}{l}{\cellcolor[HTML]{656565}\color[HTML]{FFFFFF}Improvement ideas for deriving context definitions} \\
\textbf{More diverse data} & According to one interviewee, a more diverse set of sensor data of the environment allows for easier interpretation and limitation of the context in which the system operates.\\
\rowcolor[HTML]{EFEFEF} 
\textbf{Standardised approach} & All interviewees suggested to standardised context definition to ease cooperation between different teams and companies. \\
\hline
\multicolumn{2}{l}{\cellcolor[HTML]{656565}\color[HTML]{FFFFFF}Improvement ideas for defining the ODD} \\
\textbf{Automatic tool for deriving ODD} & The described improvement would encompass a tool that can take as input the context, requirements based on the context and test cases. It would then propose an appropriate ODD, that is valid in the desired context, entails all requirements, and is verified through test cases. \\
\rowcolor[HTML]{EFEFEF}
\textbf{Clear completeness criteria for ODD} & One interviewee suggested that an explicit method and criteria are needed to proof that the ODD is complete and correct. \\
\textbf{Information should be described clearly in ODD} &  The ODD should contain more information about the context of the system. According to one interviewee, this would improve identifying wrong assumptions about the context early. \\
\rowcolor[HTML]{EFEFEF}
\textbf{Measure of exposure to a safety event} & One interviewee explained that the hazard and risk assessment to evaluate the dimensions of the ODD from a safety viewpoint. The HARA includes assumptions about the context, and especially the exposure to a hazardous context can then be used to decide on the ODD. \\
\textbf{Standardised approach} & All interviewees suggest to improve the standardisation for defining ODD. \\
\hline
\multicolumn{2}{l}{\cellcolor[HTML]{656565}\color[HTML]{FFFFFF}Improvement ideas for the process and communication} \\
\rowcolor[HTML]{EFEFEF}
\textbf{Better continuous improvement} & Automatic driving is a new technology, which needs to evolve continuously. The processes for deriving relevant artefacts, such as the context definition and ODD need to evolve together with the technology. \\
\textbf{Faster feedback} & One suggested improvement was to derive requirements faster, and creating faster feedback loops between the stakeholders. This expedites also the definition of the context, because assumptions can be made and verified faster. \\
\rowcolor[HTML]{EFEFEF}
\textbf{Improve leveraging from other contexts} & Typically automatic driving systems are developed for and tested in confined areas, such as factory areas or harbours. Lessons are learnt in these confined contexts, and it is important to be able to leverage the knowledge from these confined contexts into new contexts. \\
\textbf{Improved integration into SAFe setup} & It is perceived that requirement engineering is not well integrated in scaled agile frameworks (SAFe), which hinders an efficient development and handling of requirements, and consequently context definitions.\\
\rowcolor[HTML]{EFEFEF}
\textbf{Involvement of function developers} & Function developers should be more involved in the requirement engineering process, including context definition and deriving the ODD. On one hand, the function developers would get a better understanding of the requirements and context. On the other hand, they can contribute with deep knowledge about the used technologies, which eases the understanding of the the technology's capability for desired contexts. \\
\hline
\end{tabular}
\end{table}
\FloatBarrier

==> figure/_archive/REvsArchi.tex <==
\subsubsection{Defining the scope of the system}




as illustrated in Figure \ref{fig:03_ArchivsRE}. In fact, the proposed decomposition into several levels of abstractions can only be facilitated through requirement engineering: Starting with the stakeholders and their goals and use cases, \emph{requirements elicitation} identifies the necessary clusters of concerns of the architectural framework. \emph{Requirements interpretation} provides high level requirements necessary to fulfil the knowledge and analytical level. The resulting system and context description serve as input to the \emph{requirements negotiation}, which in turn identifies dependencies between the system's components. The dependencies are required for designing the system on the conceptual level. The resulting system specification must be reflected in the \emph{requirements documentation}, which at the same provide input to the concrete system design at the design level. The resulting solution specification needs to be validated in the \emph{requirements validation}. Because it can (and will) happen that certain requirements for AI systems cannot be validated before the system actually is deployed \cite{Bernardi2019} \martin{Find some more references here}, some requirements can only be fulfilled through behaviour monitors that report the system's behaviour and performance during run time. The data collected from the monitors at run time serve as input to the \emph{requirements management}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/System Design vs RE.pdf}
    \caption{Interaction between the architectural framework and requirement engineering\eric{I think the two columns are not on the same level. The activities on the right are independent from the abstraction level. It should be on an orthogonal axis. Perhaps the items on the arrows could go in the boxes on the right?} \martin{Good point! Maybe exchange the content of the boxes with the captions of the arrows?}}
    \label{fig:03_ArchivsRE}
\end{figure}

==> figure/_archive/RQ1.tex <==
\subsection{Exploring contextual definitions}
The following section will explore the answers given on our research questions related to contextual definitions. 
\subsubsection{RQ1: Which current solution work well for deriving contextual definitions for AI systems?}
From the interviews nine distinct themes were identified of solutions that work well when deriving contextual definition. 

\begin{table*}[t]
\centering
\caption{RQ1: Current solution working well for deriving contextual definitions for AI systems}
\label{tab:Participants}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{{m{0.2\textwidth}m{0.65\textwidth}c}}
\hline
\rowcolor[HTML]{C0C0C0}
\multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Theme}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Description}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Validated}} \\ \hline
Use cases as communication tool&All participants see use cases as an effective communication tool, even for communicating the context of the use case. However, it is difficult to argue for completeness and correctness of the use case.&\checkmark \\
\rowcolor[HTML]{EFEFEF} 
\\Simulations & Simulations are used to test efficiently various scenarios (context variations). One interview mentioned it the most cost-effective mean of testing different complex scenarios for automatic driving systems.&\checkmark \\
\\ Iterative process and feedback loops & It was stated that contextual definitions for requirements are added in an iterative process with feedback loops in which the customer regularly learns about the features of the system and can adjust the desired context accordingly. & \checkmark
\rowcolor[HTML]{EFEFEF} 
\\Test first and build an hierarchy of priorities based on lessons learned& This exploratory approach towards requirements has been described by one interviewee as a successful mean to also identify to desired and possible context of the system. & \checkmark
\\Traceability & 
\rowcolor[HTML]{EFEFEF} 
\\
\\
\rowcolor[HTML]{EFEFEF} 
\\
\\
\rowcolor[HTML]{EFEFEF} 
\\
\\
\rowcolor[HTML]{EFEFEF} 
\\
\\

\hline
\end{tabular}
\end{table*}


\subsection{RQ2: What are the challenges with deriving contextual definitions and contextual requirements from use cases?}

\subsection{RQ3: Which support would be appropriate for deriving contextual definitions and contextual requirements from use cases?}


\begin{itemize}
    \item RQ1: Current solutions
    \item RQ2: Challenges
    \item RQ3: Support
    \item Validation
\end{itemize}

==> figure/include/backmatter/A1_InterviewGuide.tex <==
\chapter{Interview guide}
\label{appendix:interview-guide}
This appendix shows the interview guide that was used for conducting the interviews.

\section*{About us}
Oskar Jakobsson \& Zuzana Rohacova \\
Studying Software Engineering Master at Chalmers.\\
Currently doing our master thesis on “Requirement representation for safety-critical and fairness aware automotive perception systems”

\section*{Purpose of Study}
The purpose of this study is to investigate challenges and current practices in requirements representation for safety-critical automotive perception systems. Specifically, for safety and fairness requirements. The goal of this interview is to get your personal experience and knowledge regarding the topic and to get insight into potential solutions. 

\section*{Starting Questions}
(10 minutes)

\subsection*{General Questions}

\textbf{Interviewee data}
\begin{itemize}
    \item What is your role in the company?
    \begin{itemize}
        \item Describe shortly your role and what you work with?
        \item How much relevant experience in years do you have with the development of perception systems in the automotive industry?
        \item Are you working in management or in development?
        \item Do you or did you actively develop software? 
    \end{itemize}
    \item Would you say that you are working mainly in research or in production / product development?
    \item What is your current relationship with requirements engineering in your company? For example, do you facilitate and define requirements or do you receive and apply them in development?
\end{itemize}

\textbf{Company data}
\begin{itemize}
    \item In which markets in the world is the company active? 
    \item Approximately, how many people work at your company?
    \item If your company works with suppliers, in which country/regions are they located? 
    \item Where is your company situated in the automotive supply chain?
    \begin{itemize}
        \item OEM
        \item Tier 1 (supplies product directly to OEM) 
        \item Tier 2 (supplies Tier 1) 
        \item Others: Specify.
    \end{itemize}
\end{itemize}

\subsection*{Terms and Concepts}
\begin{itemize}
    \item Define the following terms and concepts and ask if the interviewee agrees with the definition: 
    \begin{itemize}
        \item Non-functional requirements,
        \item ML-component, 
        \item Safety-critical systems,
        \item Fairness requirements, 
        \item Perception systems, 
        \item Related system or component (Sensors etc),
        \item Reference architecture
    \end{itemize}
\end{itemize}

\section*{Requirement representation}
(10 minutes)
\begin{itemize}
    \item In your work do you work with functional requirements for perception systems or related systems/components?
    \begin{itemize}
        \item If they say no: How do they specify desired behavior?
        \item If they say yes: Do they follow any standardized process for RE, such as those defined in ISO 26262 (for example SPICE software ..)?
        \item If they say yes: How do you represent functional requirements for perception systems or related systems/components?
        \item If they do not work directly with perception systems, what related system do they work with?
    \end{itemize}

    \item What typical non-functional requirements do you get into contact with?
    \begin{itemize}
        \item Can you rank them from the most to least important? (If not working with NFR then include slide with examples)
    \end{itemize}

    \item How do you represent non-functional requirements for perception systems or related systems/components? For example use cases, ODD, natural language...
    \begin{itemize}
        \item How do you represent the top 2 ranked requirements?
    \end{itemize}
    
\end{itemize}

\section*{Multi-party collaboration}
(10 minutes)
\begin{itemize}
    \item How do you communicate functional and non-functional requirements for perception systems within your company?
    \begin{itemize}
        \item What works well?
        \item What does not work well?
    \end{itemize}
    
    \item How do you communicate functional and non-functional requirements for perception systems with other companies in your supply chain?
    \begin{itemize}
        \item Are you using the same methods as within your company or do you use methods from another company in your supply chain?
        \item How do you figure which requirements representation to use between companies?
        \item What works well?
        \item What does not work well?
    \end{itemize}
\end{itemize}

\section*{Machine learning specific challenges}
(10 minutes)
\begin{itemize}
    \item In a nutshell, how do you approach the integration of training data in your development process for perception systems?
    \item Do you see any challenges in representing requirements both functional and non-functional because of the introduction of  ML components in the perception systems?
    \begin{itemize}
        \item If additional challenges: What are or could be, in your opinion, potential solutions to these challenges?
        \item Are there any additional non-functional requirements due to the introduction of ML-components?
            \begin{itemize}
                \item If not working with fairness: Do you see any reason or benefit in defining fairness requirements for your systems?
            \end{itemize}
        \item Did the representation of both functional and nonfunctional requirements change because of the introduction of ML-components for your company?
        \item How do you represent non-deterministic requirements for ML-components?
    \end{itemize}
\end{itemize}

\section*{Potential solutions}
(5 minutes)
\begin{itemize}
    \item Do you think a common language between all companies in the supply chain could help alleviate the identified challenges of communicating requirements and requirements representation? 
    \begin{itemize}
        \item If yes, how? If not, why not?
    \end{itemize}

    \item Do you think it is possible to have a clearly defined reference architecture for the perception systems across multiple companies in the automotive supply-chain? 
    \item Do you think it would help working with and defining requirements across multiple companies in the automotive supply chain?
\end{itemize}

\section*{Wrap-up questions}
(5 minutes)
\begin{itemize}
    \item Is there anything important that you felt we missed? Any question or subject that would be relevant to the topic (of requirement representations in multi-party automotive system development)?
    \item Do you have any person in mind (from your organisation or outside of your organisation) that we should interview as well?  
\end{itemize}






==> figure/include/backmatter/A2_MIRO_work.tex <==
\chapter{Identified themes after coding}
\label{appendix:themes_draft}

Figure~\ref{fig:themes1} and Figure~\ref{fig:themes2} show the first version of identified themes. Green boxes mark section, blue boxes mark theme and purple boxes marks comments. 

\begin{figure}[htpb]
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=1\linewidth]{figure//Methods/themes1.jpg}
    \caption{First version of identified themes}
    \label{fig:themes1}
\end{figure}

\begin{landscape}
\begin{figure}[htpb]
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=1\linewidth]{figure//Methods/themes2.jpg}
    \caption{First version of identified themes, cont'd}
    \label{fig:themes2}
\end{figure}
\end{landscape}

==> figure/include/backmatter/A3_code_categories.tex <==
\chapter{Identified categories and sub-themes from data coding}
\label{appendix:identified_categories}

Table~\ref{tab:codes} shows identifies sub-themes for each category.

%\begin{landscape}
\begin{table}[htpb]
\resizebox{\textwidth}{!}{\begin{tabular}{lll}
\textbf{Category}            & \textbf{Sub-category}                              & \textbf{Sub-theme}                          \\ \hline
Requirements representation: &                                             &                                                \\
                             & Functional requirements representation:     & FR experience                                  \\
                             &                                             & FR challenges                                  \\
                             &                                             & FR representation strategy                     \\
                             &                                             & FR comments                                    \\
                             &                                             & Following standards                            \\
                             & Non-functional requirements representation: & NFR experience                                 \\
                             &                                             & NFR challenges                                 \\
                             &                                             & NFR representation strategy                    \\
                             &                                             & NFR practices                                  \\
                             &                                             & NFR comments                                   \\ \hline
Multi-party collaboration:   &                                             &                                                \\
                             & Incompany collaboration process:            & Incompany process description                  \\
                             &                                             & Incompany challenges                           \\
                             &                                             & Incompany requirements representation          \\
                             &                                             & What works well incompany                      \\
                             & Multi-party collaboration process:          & Multiparty process description                 \\
                             &                                             & Multiparty challenges                          \\
                             &                                             & Multiparty requirements representation         \\
                             &                                             & What works well multiparty                     \\ \hline
ML challenges:               &                                             &                                                \\
                             &                                             & Approach to integration training               \\
                             &                                             & Representing ML requirements                   \\
                             &                                             & Additional challenges due to ML                \\
                             &                                             & Additional requirements due to ML introduction \\
                             &                                             & Potential solutions for ML challenges          \\ \hline
Fairness requirements:       &                                             &                                                \\
                             &                                             & How beneficial                                 \\
                             &                                             & Relation to safety                             \\ \hline
Potential solutions:         &                                             &                                                \\
                             & Common language:                            & Advantages                                     \\
                             &                                             & Challenges                                     \\
                             &                                             & Comments                                       \\
                             & Reference archietcture:                     & Advantages                                     \\
                             &                                             & Challenges                                     \\
                             &                                             & Comments                                      
\end{tabular}
}
\centering
\captionsetup{justification=centering}
\caption{Identified sub-themes from data coding }
\label{tab:codes}
\end{table}
%\end{landscape}

==> figure/include/backmatter/A4_identified_themes.tex <==
\chapter{Challenges and approaches that work well}
\label{appendix:identified_themes}
This Appendix contains a figure mapping out all the challenges and approaches that work well that were identified through thematic analysis of interviews, see Figure~\ref{identified_themes}.
\begin{landscape}
\begin{figure}[htbp]
\captionsetup{justification=centering}
\includesvg[width=\pdfpagewidth]{figure/Results/identified_themes.svg}
\caption{Identified challenges and approaches that work well}
\label{identified_themes}
\end{figure}
\end{landscape}



==> figure/include/backmatter/Lastpage.tex <==
% CREATED BY MAGNUS GUSTAVER, 2020
\newpage

%Header Last Page
\vtop{
    \null\vspace{-47.5mm}
    \centerline{\textcolor{thesisHeaderColor}{\rule{1.28\textwidth}{28mm}}}
    \null\vspace{-9mm}
    \centerline{\textcolor{headerBrown}{\rule{1.28\textwidth}{4pt}}}
    \vspace{187mm}
    \if\ThesisType M
    \centerline{\includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/AvancezChalmersU_black_centered.eps}}
    \fi
    \if\ThesisType B
    \centerline{\includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/AvancezChalmers_black_centered.eps}}
    \fi
    \vspace{-220mm}
}

\addtolength{\voffset}{2cm}
\renewcommand{\familydefault}{\sfdefault} \normalfont % Set cover page font
\pagestyle{empty}
\vspace*{-4.3cm}
\noindent
\textcolor{white}{\footnotesize \textbf{Department of Computer Science and Engineering}\\
\textbf{CHALMERS UNIVERSITY OF TECHNOLOGY} \\
Gothenburg, Sweden \\
\href{www.chalmers.se}{\textcolor{white}{www.chalmers.se}}}



==> figure/include/backmatter/References.tex <==
% CREATED BY MAGNUS GUSTAVER, 2020

\bibliographystyle{ieeetr} 
\bibliography{references} 


==> figure/include/frontmatter/Abstract.tex <==
% CREATED BY MAGNUS GUSTAVER, 2020
Requirement representation for safety-critical and fairness aware automotive perception systems\\
Identifying representation challenges for cross company collaboration\\
OSKAR JAKOBSSON \& ZUZANA ROHACOVA\\
Department of Computer Science and Engineering\\
Chalmers University of Technology \setlength{\parskip}{0.5cm}

\thispagestyle{plain}			% Supress header 
\setlength{\parskip}{0pt plus 1.0pt}
\section*{Abstract}
\mycomment{
//Introduction to topic, what is it? 
Automotive perception systems
Requirements engineering
RE for automotive percepion systems
difficulties of RE for ML?\\

//Purpose of the study, what did we do? 
Identify challenges, evaluate shared language\\

//Scope of study, what did we not do? 
Only concerned with bla bla\\

//Approach, how did we do it? 
Done through: Exploratory case study, Interview study\\


//Results, what were the outcomes? 
Lack of industry standards,
Lack of causality,
Natural language is good,
some other stuff is good\\

//Conclusions, what conclusions can we draw from the outcomes? 
Industry standards are needed (they are on their way)
Fairness is not defined
More stuff (look at conclusion chapter)\\
}

\textbf{Background:} Advancements in the field of machine learning (ML), have unlocked new capabilities for Driving Automation Systems (DAS). These DAS systems rely on the input from automotive perception systems. These systems exist in a safety-critical domain, and well-defined requirements are key to ensure that they can operate safely. However, requirements engineering (RE) for ML-enabled systems has been identified as a challenge in research. \textbf{Aim:} The thesis aimed to investigate current approaches in RE for automotive perception systems, and identify what challenges exist and which processes work well. Specifically, approaches for requirement representations, model kinds, templates, and structures. The thesis also wanted to explore if a shared language, in regards to domain description, reference system architecture, and reference information model, could help mitigate potential challenges without hindering approaches that work well. \textbf{Methods:} An exploratory case study was conducted by interviewing experts in the automotive field. This included participants from a major automotive OEM, suppliers to said OEM and experienced researchers in the automotive field. In total ten interviewees were consulted. \textbf{Results:} The challenges and what works well in the current processes in the case study companies were identified through thematic analysis of the interview data. The thesis explored the potential of a shared language to mitigate these challenges by discussing the topic with interviewees and observing brainstorming workshops for the creation of the shared language. \textbf{Conclusions:} The thesis shows that there is a lack of industry standards in RE for ML-enabled automotive perception systems, which complicates multi-party development. According to interviewees, the shared language has potential to alleviate the identified challenges. However, the feasibility of the shared language is still unclear. 


% KEYWORDS (MAXIMUM 10 WORDS)
\vfill
Keywords: Requirements engineering, requirements, perception systems, thesis, requirements representation, safety-critical, multi-party development, Automotive, shared language.

\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}

==> figure/include/frontmatter/Acknowledgements.tex <==
% CREATED BY MAGNUS GUSTAVER, 2020
\thispagestyle{plain}			% Supress header
\section*{Acknowledgements}
\mycomment{
\begin{itemize}
    \item Supervisors
    \item FAMER
    \item Participants
    \item Examiner
\end{itemize}
}


We would like to thank our supervisors, Hans-Martin Heyn and Hina Saaeda for their continued support and valuable feedback throughout the thesis. Their vast knowledge and expertise has been incredibly helpful. We would like to thank all members of the FAMER project who helped guide us in our study. We would also like to extend our deepest appreciation to the participants of the interview study, who took time out of their day to share their experience and expertise. A final thanks to our examiner Birgit Penzenstadler for evaluating our thesis and giving valuable feedback. \\

\hfill
Oskar Jakobsson \& Zuzana Rohacova, Gothenburg, May 2024

\vspace{1.5cm}
A personal thanks to my partner Ida, for unending emotional support throughout my academic journey. I am blessed to have you in my life. \\

\hfill
Oskar Jakobsson, Gothenburg, May 2024 \\


I want to thank my friends and family for their support in my academic journey.

\hfill
Zuzana Rohacova, Gothenburg, May 2024\\




\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}

==> figure/include/frontmatter/Nomenclature.tex <==
% Created by Kyriaki Antoniadou-Plytaria, 2021
\thispagestyle{plain}			% Supress header

\chapter*{Nomenclature}
Below is the nomenclature of indices, sets, parameters, and variables that have been used throughout this thesis.
% \vspace*{-3cm}

\section*{Indices}
\renewcommand*{\arraystretch}{1.35}
\begin{longtable}{p{3cm}p{12cm}}
$i$,$j$ & Indices for distribution network buses\\
$t$ & Index for time step\\
\end{longtable}

% \vspace*{-3cm}
\section*{Sets}
\renewcommand*{\arraystretch}{1.35}
\begin{longtable}{p{3cm}p{12cm}}
$\mathcal{D}$ & Set of distribution network buses\\
$\mathcal{D}_{s}$ & Set of substation buses \\
$\mathcal{H}$ & Set of time steps (simulation/scheduling horizon)\\
$\mathcal{N}$ & Set of buses\\
\end{longtable}

\section*{Parameters}
% \vspace*{-3cm}
\renewcommand*{\arraystretch}{1.35}
\begin{longtable}{p{3cm}p{12cm}}
$\gamma$& Penalty coefficient\\
$\Delta t$& Time discretization step (time interval)\\
$\eta_{j}^{ch}$& Charging efficiency of BES\\
$\eta_{j}^{dis}$& Discharging efficiency of BES\\
$\boldsymbol{H}$& Adjacency matrix\\
$N$ & Number of iterations\\
$P_{j,t}^{L}$& Active power of load demand\\
$P_{j,t}^{PV}$& Active power from solar generation\\
\end{longtable}

\section*{Variables}
\renewcommand*{\arraystretch}{1.35}
\begin{longtable}{p{3cm}p{12cm}}
$p_{j}$& Active power injection at bus $j$\\
$p_{ji}$& Active power flow from bus $j$ to bus $i$\\
$v_{i}$ & Square of voltage magnitude at bus $i$\\

\end{longtable}

\renewcommand*{\arraystretch}{1}

% \newpage				% Create empty back of side
% \thispagestyle{empty}
% \mbox{}





==> figure/include/frontmatter/Titlepage.tex <==
% CREATED BY MAGNUS GUSTAVER, 2020

\ifx\ThesisType\undefined
Undefined Thesis type in settings.tex
\else
  \if\ThesisType M
    \else
    \if\ThesisType B
    \else
    Define \textbackslash ThesisType as M for master's thesis or B for bachelor thesis in settings.tex
    \fi
  \fi
\fi

% COVER PAGE
\begin{titlepage}
\newgeometry{top=3cm, bottom=1cm,
			left=2.25 cm, right=2.25cm}	% Temporarily change margins		
			
%Header Front Page
\ifx\ThesisType\undefined
\else
    \if\ThesisType M
    \vtop{
        \null\vspace{-25mm}
        \centerline{\includegraphics[width=1.18\textwidth]{figure/auxiliary/GrayHeaderPattern.jpg}}
        \vspace{-2.3cm}
        \hbox{\hspace{0mm}\includegraphics[height=18mm]{figure/auxiliary/AvancezChalmersU_white_right.eps}}
        \centerline{\textcolor{headerBrown}{\rule{1.18\textwidth}{4pt}}}
        \vspace{\paperheight}\vspace{-85mm}
        \centerline{\textcolor{thesisHeaderColor}{\rule{1.1\textwidth}{0.8pt}}} % Rule after Department
        \vspace{-\paperheight}\vspace{85mm}
    }
    \fi
    \if\ThesisType B
    \vtop{
        \null\vspace{-25mm}
        \centerline{\includegraphics[width=1.18\textwidth,height=80pt]{figure/auxiliary/GreenHeaderPattern.jpg}}
        \vspace{-2.3cm}
        \hbox{\hspace{0mm}\includegraphics[height=18mm]{figure/auxiliary/AvancezChalmers_white_right.eps}}
        \centerline{\textcolor{headerBrown}{\rule{1.18\textwidth}{4pt}}}
        \vspace{\paperheight}\vspace{-85mm}
        \centerline{\textcolor{thesisHeaderColor}{\rule{1.1\textwidth}{0.8pt}}} % Rule after Department
        \vspace{-\paperheight}\vspace{85mm}
    }
    \fi
\fi

% Cover picture (replace with your own or delete)		
%\begin{figure}[H]
%\centering
%\vspace{1cm}	% Adjust vertical spacing here
%\includegraphics[width=0.7\linewidth]{figure/Wind.png}
%\end{figure}

% Cover text
\mbox{}
\vfill
\renewcommand{\familydefault}{\sfdefault} \normalfont % Set cover page font
\textbf{{\Huge 	Requirement representation for safety-critical
                and fairness aware automotive perception systems}} 	\\[0.5cm]
{\Large Identifying requirements representation challenges for multi-party collaboration.}\\[0.5cm]
Master's thesis in Software engineering and technology \setlength{\parskip}{1cm}

\noindent
{\Large OSKAR JAKOBSSON} \setlength{\parskip}{1.5cm} \\
{\Large ZUZANA ROHACOVA} \setlength{\parskip}{1.5cm}

\noindent
\textcolor{thesisHeaderColor}{\small\textbf{DEPARTMENT OF COMPUTER SCIENCE AND ENGINEERING}}
\setlength{\parskip}{1mm}

\textsc{Chalmers University of Technology} \\
{\small Gothenburg, Sweden \the\year \\
\href{www.chalmers.se}{www.chalmers.se}}\vspace{1.7cm}

\renewcommand{\familydefault}{\rmdefault} \normalfont % Reset standard font
\end{titlepage}


% BACK OF COVER PAGE (BLANK PAGE)
\newpage
\restoregeometry
\thispagestyle{empty}
\mbox{}


% TITLE PAGE
\newpage
\thispagestyle{empty}
\begin{center}
	\textsc{\large Master's thesis \the\year}\\[4cm]
	\textbf{\Large Requirement representation for safety-critical and fairness aware automotive
perception systems} \\[1cm]
	{\large Identifying requirements representation challenges for multi-party collaboration}\\[1cm]
	{\large OSKAR JAKOBSSON} \\
        {\large ZUZANA ROHACOVA}
	
	\vfill	
	% Logotype on titlepage	
	\begin{figure}[H]
	\centering
	% Remove this figure to remove the titlepage logotype
	\if\ThesisType M
    \includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/AvancezChalmersU_black_centered.eps} \\
    \fi
    \if\ThesisType B
    \includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/AvancezChalmers_black_centered.eps} \\
    \fi
	%\includegraphics[width=0.2\pdfpagewidth]{figure/auxiliary/AvancezChalmersU_black_centered.eps} \\
	\end{figure}	\vspace{5mm}	
	
	Department of Computer Science and Engineering \\
	\textsc{Chalmers University of Technology} \\
	Gothenburg, Sweden \the\year \\
\end{center}


% IMPRINT PAGE (BACK OF TITLE PAGE)
\newpage
\thispagestyle{plain}
\vspace*{4.5cm}
Requirement representation for safety-critical and fairness aware automotive perception systems\\
Identifying requirements representation challenges for multi-party collaboration\\
OSKAR JAKOBSSON \setlength{\parskip}{1cm}
ZUZANA ROHACOVA \setlength{\parskip}{1cm}

\copyright ~ OSKAR JAKOBSSON, \the\year. \setlength{\parskip}{1cm}\\
\copyright ~ ZUZANA ROHACOVA, \the\year. \setlength{\parskip}{1cm}

Supervisor: Hans-Martin Heyn, and Hina Saeeda Department of Computer Science and Engineering\\
Examiner: Birgit Penzenstadler, Department of Computer Science and Engineering \setlength{\parskip}{1cm}

Master's Thesis \the\year\\	
Department of Computer Science and Engineering\\
Chalmers University of Technology\\
SE-412 96 Gothenburg\\
Telephone +46 31 772 1000 \setlength{\parskip}{0.5cm}

\vfill
% Caption for cover page figure if used, possibly with reference to further information in the report
\setlength{\parskip}{0.5cm}

Typeset in \LaTeX \tagtemp\\
Printed by Chalmers Reproservice\\
Gothenburg, Sweden \the\year


==> figure/include/frontmatter/acronyms.tex <==
% Created by Kyriaki Antoniadou-Plytaria, 2021
\thispagestyle{plain}			% Supress header
% \vspace*{3.5cm}
% \section*{List of Acronyms}
\chapter*{List of Acronyms}
Below is the list of acronyms that have been used throughout this thesis listed in alphabetical order:
\vspace*{1.0cm}

%\begin{table}[H]
%\centering
\begin{tabular}{p{3cm}p{12cm}}
BES & Battery Energy Storage\\
DER & Distributed Energy Resource\\
MILP & Mixed-Integer Linear Programming\\
MG & Microgrid \\
PV & Photovoltaic\\
RES & Renewable-based Energy Sources\\
\end{tabular}
%\end{table}


\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}



==> figure/include/settings/Settings.tex <==
% CREATED BY Kyriaki Antoniadou-Plytaria, 2021

% BASIC SETTINGS
\usepackage{svg}
\usepackage{moreverb}								% List settings
\usepackage{textcomp}								% Fonts, symbols etc.
\usepackage{lmodern}								% Latin modern font
\usepackage{helvet}									% Enables font switching
\usepackage[T1]{fontenc}							% Output settings
\usepackage[english]{babel}							% Language settings
\usepackage[utf8]{inputenc}							% Input settings
\usepackage{amsmath}								% Mathematical expressions (American mathematical society)
\usepackage{amssymb}								% Mathematical symbols (American mathematical society)
\usepackage{graphicx}								% Figures
\usepackage{subfig}									% Enables subfigures
\numberwithin{equation}{chapter}					% Numbering order for equations
\numberwithin{figure}{chapter}						% Numbering order for figures
\numberwithin{table}{chapter}						% Numbering order for tables
\usepackage{listings}								% Enables source code listings
\usepackage{chemfig}								% Chemical structures
\usepackage[top=3cm, bottom=3cm,
			inner=3cm, outer=3cm]{geometry}			% Page margin lengths			
\usepackage{eso-pic}								% Create cover page background
\newcommand{\backgroundpic}[3]{
	\put(#1,#2){
	\parbox[b][\paperheight]{\paperwidth}{
	\centering
	\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
\usepackage{float} 									% Enables object position enforcement using [H]
\usepackage{parskip}								% Enables vertical spaces correctly 

\newcommand{\mycomment}[1]{}
\usepackage{soul}

% To rotate images
\usepackage{pdflscape}

% DEFINE THESIS TYPE
\def\ThesisType{M} % M - master, B - bachelor

% COLOR FOR HEADERS
\definecolor{headerBrown}{RGB}{144,102,78}
\if\ThesisType B
\definecolor{thesisHeaderColor}{RGB}{126,180,56} % Green
\fi
\if\ThesisType M
\definecolor{thesisHeaderColor}{cmyk}{0.14,0,0,0.65} % Gray
\fi

% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)

% Disable automatic indentation (equal to using \noindent)
\setlength{\parindent}{0cm}                         


% Caption settings (aligned left with bold name)
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{caption} 		

		  	
% Activate clickable links in table of contents  	
\usepackage{hyperref}								
\hypersetup{colorlinks, citecolor=black,
   		 	filecolor=black, linkcolor=black,
    		urlcolor=black}

% To be able rotate images
\usepackage{rotating}

% Define the number of section levels to be included in the t.o.c. and numbered	(3 is default)	
\setcounter{tocdepth}{5}							
\setcounter{secnumdepth}{5}	


% Chapter title settings
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]


% Header and footer settings (Select TWOSIDE or ONESIDE layout below)
\usepackage{fancyhdr}								
\pagestyle{fancy}  
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\space#1}{}} 


% Select one-sided (1) or two-sided (2) page numbering
\def\layout{2}	% Choose 1 for one-sided or 2 for two-sided layout
% Conditional expression based on the layout choice
\ifnum\layout=2	% Two-sided
    \fancyhf{}			 						
	\fancyhead[LE,RO]{\nouppercase{ \leftmark}}
	\fancyfoot[LE,RO]{\thepage}
	\fancypagestyle{plain}{			% Redefine the plain page style
	\fancyhf{}
	\renewcommand{\headrulewidth}{0pt} 		
	\fancyfoot[LE,RO]{\thepage}}	
\else			% One-sided  	
  	\fancyhf{}					
	\fancyhead[C]{\nouppercase{ \leftmark}}
	\fancyfoot[C]{\thepage}
\fi


% Enable To-do notes
\usepackage[textsize=tiny]{todonotes}   % Include the option "disable" to hide all notes
\setlength{\marginparwidth}{2.5cm} 


% Supress warning from Texmaker about headheight
\setlength{\headheight}{15pt}		


% Tag command (invisible)
\newcommand{\tagtemp}{\textcolor{white}{, template by Kyriaki Antoniadou-Plytaria}}

% Allow a table to split
\usepackage{longtable}

\usepackage[listings]{tcolorbox}%





==> figure/include/temp_notes.tex <==
% I1: Shared language always helps. Not sure how to create one "here". People do still interprete differently but still helps alot. Difficult to define and create.

% I2:
% - Yeah, I I definitely think so. 
% -  not any common language and also it's always like you know a barrier at the first proof of concept for a new guideline to align on all of these things. 

% I3:
% -yes, even if its a bad solution
% - , the first challenge is traceability of the requirements and if the parties they define the requirements in different ways. - to have consensus on the common language

% I4: 
% - yes

% I5: 
% - for sure
% - tried, works in some cases

% I6:
% -yes
% - So we have bigger challenge to solve actually maybe sometimes when we have identified some of the issues then we could come to this common challenge common language challenge when we know what we are going to achieve. What here is like something is missed like a we we could not make good connection in this like from a OEM to us
% - time for it should be later

% I7:
% - I think right now we have quite a good development within the operational design domain. 
% - I think people are  getting more understanding of what it is and that is something communicable and all the companies know what it is.
% - communicate between the different companies using the machine readable format which is based on the open scenario standard so that that is something. OEMS, and every other companies working on and so and I think that that is what's happening now. 

% I8:
% - Yeah, I yeah, I I agree to this one because the standard doesn't mention how you should write the requirements. And every company interprets in a different way.
% - I suppose as long as it's not ambiguous, that's important, but having some kind of a framework doesn't. It will do good, especially when working with suppliers. 

% I9: 
% Yes, and in many ways I do believe this exists. For example in terms of ML terminology, generally speaking people mean the same thing when they say precision, recall, etc. It's always confusing when you have different words for similar situations.

----------------------RA
% I1: Solution space is too big, will be difficult to have it well defined. It would definitely be effective but depending on how specific it may not be possible. (It may be possible if it is done on a high level)

% I2:
% -would be good but hard to see it happening
% - giving too much information to other companies (companies in supply chai would not really like that, scared to sell companies information)
% - would be helpful, as the communication is now needed to ask hat is what

% I3:
% - I don't think it will be possible.
% - it will be 1 system, one product, not every company will follow that.
% - there are some examples before that, the whole industry decided on one main architecture to basically make it simple for themselves to argue for safety. And this kind of stuff, they decided on one architecture and used that. But I think it is not feasible, at least at the moment where we are right now. Maybe in near future everybody agree on one, yeah. 
% - Uh, because everybody thinks that they have the best ever solution. That's one thing. The second thing is that there is so much secrecy around this stuff. 
% - releasing architecture is cheaper to develop
% - Easier? Not necessarily, but It can lead to better requirements because it's not easy, because then instead of you and your colleagues in the OEM and maybe your suppliers, you need to, uh, discuss it with so many other parties. 

% I4: 
% - I think it I think it's possible. But again, I think it can be even more general.
% - The perception system on camera would probably be organized in the same way when it comes to artificial intelligence or ML. You need the same principles. 
% - So they call it  trucks. So it's a different different set, but they also share a a common set of safety goals. So that's one example that we could potentially do and it's related to this as well, so. 
% - we have different owners previously and I think it was hard to align some parts, I don't know when we say reference architecture is that a set of principles or yeah that would be like or is it also like...  
% -  you define a third which both and which both enterprises can connect to, and you like a common reference point. And each of these enterprises, they know what this means in my context

% I5:
% - I think more or less they do because the architecture is more or less defined by the tier ones. Uh it depends on the on the top level architecture is on the OEM, but if you're talking about OK, I need this integrated system that they talk about. 
%  - cant really, every manufacturer wants to be unique
% - it would help with tailoring requirements

% I6:
% - used to be trend, but now with ML systems
% For a black box nature of an AI system, like if you have an AI system that as an input it has like sensors and then different layer of like with 1000 nodes in each layer and then it's acting, can we define an architecture for that giant components ML component if if it's possible then that's stuck. 
% - I mean, no matter if we don't have requirements or not in some way, we need to be able to understand each other through this supply chain.
% -we should know why we are doing it a specific task every like involving and organization in the supply chain should know or should have a common understanding about why they are doing a certain type of action or certain type of there requirements or expectations from each other

% I7:
% - So, I think at the very high level you have reference architecture which is pretty straightforward. But when you're going down to the lower level and I think that's the kind of each company's own design, it's it's individual. 
% - dont know if possible because it is complcated


% I8:
%  Have every company as of today, I suppose, use their sensors in a different way. Maybe they only wanna fuse camera and light or and not ultrasonics. You know, some companies might wanna. Yeah, fuse everything and create just one huge output. Uh, so it's different, yeah

% I9: Yes, if shared with confidentiality I suppose. However, that's pretty hard to achieve in practice. Many of our clients do not want to share too much information about their ML approach for example.
